UniBriVL: Robust Universal Representation and Generation of Audio Driven Diffusion Models

Multimodal large models have been recognized for their advantages in various performance and downstream tasks. The development of these models is crucial towards achieving general artificial intelligence in the future. In this paper, we propose a novel universal language representation learning method called UniBriVL, which is based on Bridging-Vision-and-Language (BriVL). Universal BriVL embeds audio, image, and text into a shared space, enabling the realization of various multimodal applications. Our approach addresses major challenges in robust language (both text and audio) representation learning and effectively captures the correlation between audio and image. Additionally, we demonstrate the qualitative evaluation of the generated images from UniBriVL, which serves to highlight the potential of our approach in creating images from audio. Overall, our experimental results demonstrate the efficacy of UniBriVL in downstream tasks and its ability to choose appropriate images from audio. The proposed approach has the potential for various applications such as speech recognition, music signal processing, and captioning systems.

==> table/pretext.tex <==
\subsection{Different pretext tasks}

\begin{figure}[ht]
% \vspace{-1.1em}
\centering
\includegraphics[width=\linewidth]{src/train_num.pdf}
\caption{VGGSound audio classification results with different percentage (\%) of training samples. Comparisons between Supervise, OpenL3, YamNet, and Wav2CLIP.}
\label{fig:train_num}
\vspace{-1.0em}
\end{figure}

From Figure \ref{fig:train_num}, we see results of amount of training data to train downstream classifiers on VGGSound, compared among Supervise, OpenL3, YamNet, and Wav2CLIP. Both YamNet and Wav2CLIP only require $\sim$1/10 amount of data to reach similar performance as Supervise counterpart in the smaller labeled data region, and eventually all others outperform OpenL3 when enough labels are available.

YamNet and Wav2CLIP yield very similar trend throughout all our comparisons (Table \ref{tab:all_tasks} and Figure \ref{fig:train_num}), except for FSD50K and TAU, where we hypothesize that the match between pretext and downstream tasks does affect the performance. However, this is still surprising that they perform very similarly on all other classification tasks, as the pretext tasks for pre-training are very different, while YamNet requires large amount of labeled data, Wav2CLIP is pre-trained without human annotations, and is therefore easier to scale.
